AMRFact: Enhancing Summarization Factuality Evaluation with AMR-Driven Negative Samples Generation

Ensuring factual consistency is crucial for natural language generation tasks, particularly in abstractive summarization, where preserving the integrity of information is paramount. Prior works on evaluating factual consistency of summarization often take the entailment-based approaches that first generate perturbed (factual inconsistent) summaries and then train a classifier on the generated data to detect the factually inconsistencies during testing time. However, previous approaches generating perturbed summaries are either of low coherence or lack error-type coverage. To address these issues, we propose AMRFact, a framework that generates perturbed summaries using Abstract Meaning Representations (AMRs). Our approach parses factually consistent summaries into AMR graphs and injects controlled factual inconsistencies to create negative examples, allowing for coherent factually inconsistent summaries to be generated with high error-type coverage. Additionally, we present a data selection module NegFilter based on natural language inference and BARTScore to ensure the quality of the generated negative samples. Experimental results demonstrate our approach significantly outperforms previous systems on the AggreFact-SOTA benchmark, showcasing its efficacy in evaluating factuality of abstractive summarization.

==> tables/error_typology.tex <==
\begin{table*}[h]
\small
\centering
\begin{tabular}{p{2.6cm}|p{6.4cm}|p{5.7cm}}
\toprule
\textbf{Error Type} & \textbf{Description} & \textbf{Example} \\ 
\midrule
Predicate Error & The predicate of the summary does not align with the information provided in the original document. & Hingis \textcolor{red}{\textit{ended}} a two-year ban after testing positive for cocaine at 2007 Wimbledon. \\
\midrule
Entity Error & The primary arguments, or their attributes, associated with the predicate are incorrect. & \textcolor{red}{\textit{Kournikova}} began a two-year ban after testing positive for cocaine at Wimbledon in 2007. \\
\midrule
Circumstance Error & The supplementary details, such as location or time, that define the context of a predicate are incorrect. & Hingis began a two-year ban after testing positive for cocaine at Wimbledon in \textcolor{red}{\textit{2014}}. \\
\midrule
Discourse Link Error & Errors arise from the improper connection of statements within the discourse, such as errors in temporal ordering or causal link. & Hingis began a two-year ban \textcolor{red}{\textit{before}} testing positive for cocaine at Wimbledon in 2007. \\
\midrule
Out of Article Error & The statement conveys information that is absent in the original document. & Hingis and Kournikova will team up again to play at this year's \textcolor{red}{\textit{All England Club}}. \\

\bottomrule
\end{tabular}
\caption{Typology of factual errors. Original document fragment for the examples: \textit{(CNN)  -- Martina Hingis and Anna Kournikova will team up again to play at this year's Wimbledon championships. [...] Swiss star Hingis won five grand slam singles crowns and nine in doubles during a glittering career which ended under a cloud in 2007, when she was suspended for two years for testing positive for cocaine at Wimbledon. [...]} 
\haoyi{add one row to include original document and an AMR graph for reference summary. Highlight the applied perturbations with different color to be mapped to the below examples.}
}
\label{tab:factual-errors}
\end{table*}
